Learning to Assess Danger from Movies for Cooperative Escape Planning in Hazardous Environments

There has been a plethora of work towards improving robot perception and navigation, yet their application in hazardous environments, like during a fire or an earthquake, is still at a nascent stage. We hypothesize two key challenges here: first, it is difficult to replicate such scenarios in the real world, which is necessary for training and testing purposes. Second, current systems are not fully able to take advantage of the rich multi-modal data available in such hazardous environments. To address the first challenge, we propose to harness the enormous amount of visual content available in the form of movies and TV shows, and develop a dataset that can represent hazardous environments encountered in the real world. The data is annotated with high-level danger ratings for realistic disaster images, and corresponding keywords are provided that summarize the content of the scene. In response to the second challenge, we propose a multi-modal danger estimation pipeline for collaborative human-robot escape scenarios. Our Bayesian framework improves danger estimation by fusing information from robot's camera sensor and language inputs from the human. Furthermore, we augment the estimation module with a risk-aware planner that helps in identifying safer paths out of the dangerous environment. Through extensive simulations, we exhibit the advantages of our multi-modal perception framework that gets translated into tangible benefits such as higher success rate in a collaborative human-robot mission.

==> contents/experiments.tex <==
\section{Simulations}
\label{sec:simulations}


\subsection{Environment}
\label{subsec:simEnvironment}
For simulation, we leverage the School environment from \cite{shree2021exploiting}. However, the sparse connectivity of the graph leads to very few possible paths. Thus, to introduce the possibility of more interesting navigational behaviors, we add a few more nodes to the graph and is shown in Fig.~\ref{fig:schoolGraph}. The final graph consists of a total of $n=54$ nodes. We manually assign scene characteristics e.g. fire, flood, etc., for different segments of the environment. Accordingly, to match the scene description, each node is associated with an image from the test set available from our extreme environment dataset. 

% \begin{figure}
%      \centering
%      \begin{subfigure}[b]{0.35\textwidth}
%          \centering \includegraphics[trim= 0 0 0 38, clip, width=\textwidth]{images/schoolMapExtraNodes.png}
%          \caption{\small Graph structure} \label{fig:schoolGraphStructure}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.35\textwidth}
%          \centering \includegraphics[trim= 200 50 200 100, clip, width=\textwidth]{images/schoolEnvDangerEnv3.png}
%          \caption{\small Danger map} \label{fig:schoolGraphDanger}
%      \end{subfigure}
%         \caption{Graphical representation of the environment used in our simulations. }
%         \label{fig:schoolGraph}
% \end{figure}



\begin{figure}
    \centering \includegraphics[trim= 140 100 110 70, clip, width=0.4\textwidth]{images/schoolMapNew.pdf}
    \caption{Graphical representation of the environment used in our simulations, with danger map.}
    \label{fig:schoolGraph}
\end{figure}



% \begin{figure}
%     \centering
%     \includegraphics[trim= 0 0 0 38, clip, width=0.35\textwidth]{images/schoolMapExtraNodes.png}
%     \caption{\small Graphical representation of the environment used in our simulations.}
%     \label{fig:schoolGraph}
% \end{figure}

\subsection{Danger estimation and survival probability}
\label{subsec:simDangerEstimation}
At time $t$,
the robot calculates the danger of the current and neighboring nodes with the help of our Bayesian estimation framework. \vikram{For all the non-neighboring nodes, we assume a uniform prior danger distribution.} Note that the robot does not have access to the true survival probability $s_{ij}$, needed to solve the optimization problem Eq.~\eqref{eq:shortestPathProblem}. It must rely on the danger estimate $\hat{D}$ to establish an approximation for the survival probability $\hat{s}_{ij} = p(\hat{D}\leq\tau)$, where $\tau$ is the tolerable danger level for the team. Thus, the robot optimizes for $\hat{s}^{\pi}$ and moves one step along the optimal path $\boldsymbol{\pi^{*}}$. This process keeps repeating till the robot reaches the goal node $v_{\text{node}}$.




% The survival probability $s_{ij}$ depends on the 

% To assess the survival proba


% use different modalities: vision, language, and both combined, to estimate the danger level of the current node where the human-robot is

\begin{figure*}[!ht]
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering \includegraphics[trim= 0 0 0 0, clip, width=\textwidth]{images/success_rate_planning_ver2.eps}
         \caption{\small Mission success rate} \label{fig:successRate}
     \end{subfigure}
     \begin{subfigure}[b]{0.32\textwidth}
         \centering \includegraphics[trim= 0 0 0 0, clip, width=\textwidth]{images/avg_exposure_planning_ver2.eps}
         \caption{\small Avg. number of intolerable exposures} \label{fig:exposures}
     \end{subfigure}
     \begin{subfigure}[b]{0.32\textwidth}
         \centering \includegraphics[trim= 0 0 0 0, clip, width=\textwidth]{images/average_path_planning_ver2.eps}
         \caption{\small Avg. path length} \label{fig:pathLength}
     \end{subfigure}
        \caption{Planning results: performance with different sensing modalities. Results are obtained from 1000 simulation runs.}
        \label{fig:planningResults}
\end{figure*}

\subsection{Results and Discussion}
\label{subsec:simResults}

\vikram{We perform 1000 Monte Carlo simulations of the combined planning and danger estimation framework with different sensor modalities and for different tolerable danger level $\tau$. The ``no-sensor'' case is when the robot is unable to perceive danger. The ``full-knowledge'' case refers to the hypothetical situation when the robot is aware of the danger map of the whole environment. In addition to the two performance metrics, we also show the average path length of the mission in Fig~\ref{fig:planningResults}. Note that we do not report results for $\tau=5$ since it corresponds to the unrealistic case when the team can survive even extreme danger.}   
% planning framework, along with danger estimation module with different sensor modalities and different values of tolerable danger level $\tau$. Results are presented in Table~\ref{tbl:planningPerformance}.


\vikram{
\subsubsection{Success rate}
In Fig~\ref{fig:successRate}, we observe that the ``no sensor'' case has lowest success rate amongst all methods for every value of $\tau$. This indicates that ability to perceive and account for danger is critical for mission success in disaster scenarios. 

A further analysis of different modalities provides some intriguing insights. The ``vision only'' sensing consistently outperforms ``language only'' sensing. As mentioned earlier, this is because of the richness of visual data compared to single word inputs. Interestingly, the ``vision-only'' success rate is even competitive to the multi-modal methods, implying that the perception benefits mentioned in Table~\ref{tbl:multiModalDangerResults} are not exactly translated into mission success. Nonetheless, highest success is achieved in VL-10 case by fusing information across the vision and language domain, thus, supporting our hypothesis that improved perception leads to more successful missions.
% reaps the rewards by accomplishing higher mission success rate.

\subsubsection{Average number of exposures}
As anticipated, Fig~\ref{fig:exposures} suggests that a lack of danger sensing causes highest number of hazardous exposures to the team. Occasionally, such exposures can prove fatal for the team in a real-world mission. 

Surprisingly, the average intolerable exposure for the ``full knowledge'' case is higher in case of $\tau=1$ and $2$. To understand this, we need to focus on the average path length, shown in Fig~\ref{fig:pathLength}. With full knowledge of the danger map, the robot tries to avoid the regions with high danger, causing the team to spend more time inside the environment. In contrast, when the robot has only access to local danger data, it plans myopically and the path tends to be shorter.
% to only local danger data in the map, the robot plans myopically and tends to take a shorter path to the exit.
% When the robot has full knowledge of danger map, it tries to avoid 
% Unlike the robot with full knowledge of danger, in all other cases the robot plans myopically and tends to take a shorter path to the exit. In contrast, with ``full knowledge'' the robot tries to avoid the regions with high danger, causing the team to spend more time inside the environment. 
As a consequence of the extra time spent in the hazardous environment and danger $D$ being probabilistic, the risk of getting exposed to intolerable danger increases.

The results demonstrate that for $\tau=1$ and $2$, there is at least $20\%$ reduction in hazardous exposures with the Bayesian multi-modal framework compared to other methods. For higher danger tolerances, vision-only sensing works equally well and achieves competitive exposure levels to multi-modal methods. It is interesting to note that all three multi-modal approaches i.e. VL-1, VL-5, and VL-10, yield similar average exposures, implying that having more number of words from the human did not help in this regard.
}

% \subsubsection{Varying sensor modality} 
% Clearly, with no sensor the mission success rate is the lowest and has the highest number of catastrophic failures. With vision-based danger estimation, the success rate improves by 100\% and the number of failures reduce to about half of the initial value. Furthermore, combining both vision and language achieves competitive performance to the case with ``true'' danger sensing. The results suggest that our proposed framework is able to leverage both the modalities to get a superior danger estimate and utilize it for planning a risk-aware path out of the extreme environment.
% We observe from Table~\ref{tbl:planningPerformance} that the 



% % RESULTS FOR ENV 3
% \begin{table}
% % \vspace{0.1in}
% \centering
% \caption{ \small \vikram{Performance evaluation of combined danger estimation and planning framework for the collaborative escape problem.}}
% % \tabcolsep 3.5pt
% % \begin{tabular}{|l|l|l|}
% \begin{tabular}{|p{1.9cm}|p{0.4cm}|p{2cm}|p{1cm}|p{1.2cm}|}
% \hline
%   \textbf{Modality} & $\boldsymbol{\tau}$ & \textbf{Avg. \# of intolerable exposures} & \textbf{Success rate} &\textbf{Avg. path length}\\ 
%   \hline 
%   No sensor &  2 & 3.9 & 15.9\% & 6.8\\ 
%   Full knowledge &  2 & 2.7 & 27.4\% & 9.7\\ 
%   Vision only &  2 & 3.1 & 22.2\% & 6.8\\
%   Language only & 2 & 3.2 & 20.9\% & 6.8\\
%   VL 1-word & 2 & 2.5 & 26.6\% & 7.6\\
%   VL 5-words & 2 & 2.5 & 27.9\% & 7.7\\
%   VL 10-words & 2 & 2.5 & 27.9\% & 7.9\\
%   \hline
%   No sensor &  3 & 2.7 & 19.5\% & 6.8\\ 
%   Full knowledge &  3 & 1.2 & 43.4\% & 9.5\\ 
%   Vision only &  3 & 1.4 & 41.9\% & 7.6\\
%   Language only & 3 & 2.0 & 26.2\% & 6.9\\
%   VL 1-word & 3 & 1.4 & 39.2\% & 7.7\\
%   VL 5-words & 3 & 1.4 & 43.2\% & 7.8\\
%   VL 10-words & 3 & 1.4 & 43.5\% & 8.8\\
%   \hline
%   No sensor &  4 & 1.3 & 32.5\% & 6.8\\ 
%   Full Knowledge &  4 & 0.5 & 67.5\% & 9.3\\ 
%   Vision only & 4 & 0.5 & 64.8\% & 7.6\\
%   Language only & 4 & 0.9 & 41.9\% & 6.8\\
%   VL 1-word & 4 & 0.5 & 65.0\% & 7.6\\
%   VL 5-words & 4 & 0.6 & 63.4\% & 8.4\\
%   VL 10-words & 4 & 0.6 & 65.1\% & 9.3\\  
% %   No sensor &  3 & 2.6 & 23.7\%\\ 
% %   Truth sensor &  3 & 1.0 & 52.3\%\\ 
% %   Vision only &  3 & 1.3 & 45.9\%\\
% %   Language only & 3 & 1.5 & 42.0\%\\
% %   VL 1-word & 3 & 2.3 & 36.0\% & 7.3\\
% %   VL 5-words & 3 & NA & NA\\
% %   VL 10-words & 3 & NA & NA\\

%  \hline
% \end{tabular}
% \label{tbl:planningPerformance}
% \end{table}


% \begin{figure}
%      \centering
%      \begin{subfigure}[b]{0.4\textwidth}
%          \centering \includegraphics[trim= 0 0 0 0, clip, width=\textwidth]{images/success_rate_planning_tol_1_to_4.eps}
%          \caption{\small Mission success rate} \label{fig:successRate}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.4\textwidth}
%          \centering \includegraphics[trim= 0 0 0 0, clip, width=\textwidth]{images/avg_exposure_planning_tol_1_to_4.eps}
%          \caption{\small Avg. number of intolerable exposures} \label{fig:exposures}
%      \end{subfigure}
%      \begin{subfigure}[b]{0.4\textwidth}
%          \centering \includegraphics[trim= 0 0 0 0, clip, width=\textwidth]{images/average_path_planning_tol_1_to_4.eps}
%          \caption{\small Avg. path length} \label{fig:pathLength}
%      \end{subfigure}
%         \caption{Planning results: performance with different sensing modalities. Results are obtained from 1000 simulation runs.}
%         \label{fig:planningResults}
% \end{figure}



% \subsubsection{Varying tolerable danger $\tau$}


% \vikram{To do}


